Continual Test-Time Adaptation via Entropy Sensitivity-Guidance in Strict Online Setting

Test-time adaptation (TTA) promises robustness under distribution shift by updating a pretrained model on unlabeled test data, but strict online TTA with batch size one and no access to source data is especially prone to drift or collapse. We introduce Sensitivity-Guided Erasing Adaptation (SEGA), a method for strict online continual TTA (CTTA) on corruption-style streams. SEGA uses a small number of structured erasures to probe how predictive entropy changes as information is removed, and uses the resulting per-sample sensitivity trajectories to coordinate recovery and sample selection rather than relying on raw entropy or batch statistics. This yields a practical feedback signal for long-horizon batch-size-one adaptation without periodic resets or model reservoirs. In experiments on ImageNet-C, CIFAR10/100-C, and corruption-generated aquaculture streams treated as controlled corruption-style proxies, SEGA yields consistent robustness and stability gains over strong CTTA baselines while reducing backward passes through sensitivity-based gating.

==> figures/cam_tsne.tex <==
\begin{figure*}[t!]
    \centering
    \small
    % Left: CAM (about 70%)
    \begin{minipage}[t]{0.55\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cam/cam.png}
        % Optional: sub-caption via \subcaption if you use it
        % \subcaption{GradCAM on FreshFish-C corruption samples.}
        % \label{fig:cam}
    \end{minipage}
    \hfill
    % Right: t-SNE (about 30%), 2x2 grid
    \begin{minipage}[t]{0.40\textwidth}
        \centering
        \subfigure[Source]{
            \includegraphics[width=0.3\linewidth]{figures/tsne/source.jpg}
        }
        \subfigure[$\mathcal{L}_{\mathrm{el}}$]{
            \includegraphics[width=0.3\linewidth]{figures/tsne/maskel.jpg}
        }\\[2pt]
        \subfigure[$\mathcal{L}_{\mathrm{cl}}$]{
            \includegraphics[width=0.3\linewidth]{figures/tsne/maskcl.jpg}
        }
        \subfigure[$\mathcal{L}_{\mathrm{SEGA}}$]{
            \includegraphics[width=0.3\linewidth]{figures/tsne/mask.jpg}
        }
    \end{minipage}

    \caption{Left: GradCAM visualizations on corrupted FreshFish-C samples.
    Right: t-SNE of forward features from the adapted ViT-Base on FreshFish-C
    at severity level~5 under different objectives.}
    \label{fig:cam_tsne}
\end{figure*}

==> figures/effect.tex <==
\begin{figure*}[h!]
    \centering
    \small
    \subfigure[Recovery Timeline]{
        \includegraphics[width=0.36\textwidth]{figures/problem/sega/model_reset/model_recovery.png}
    }
    \subfigure[Reset Outcomes]{
        \includegraphics[width=0.28\textwidth]{figures/problem/sega/model_reset/reset_event_heatmap.png}
    }
    \subfigure[Entropy Separation]{
        \includegraphics[width=0.29\textwidth]{figures/problem/sega/sample_filter/sample_filter.png}
    }

    \caption{SEGA effect on CTTA (batch size 1) with FreshFish-C~\citep{BiswasFishDisease2024} using ViT-Base.
    (a) Recovery timeline: rolling test error over sample steps with domain boundaries and vertical reset markers, showing when resets trigger relative to distribution shifts and how they affect the error stream.
    (b) Reset outcomes: each point is a reset event, plotting before and after reset error against the $y{=}x$ line and colored by sample step, so helpful resets (error drops) cluster below the diagonal.
    (c) Entropy separation: normalized entropy histograms for correct vs incorrect predictions with a shaded high-entropy ``unreliable'' zone and summary fractions, indicating how well entropy isolates hard, error-prone samples.}
    \label{fig:sega_effect}
\end{figure*}



==> tables/cifar100c_ctta_avg.tex <==
\begin{table*}[h!]
    \centering
    \small
    \caption{Classification error rate (\%) under CTTA (batch size 1) on CIFAR100-C using ViT-Base. Mean is the average across 15 corruption domains, each with 10000 test samples. Gain is the relative improvement over the source model. Entries report mean and standard deviation of three runs (seeds 1, 2, 3). }
    \label{tab:cifar100c_tta_continual_avg}
    \setlength\tabcolsep{6pt}
    \resizebox{\linewidth}{!}{%% relies only on graphicx, already loaded by bmvc2k
    \begin{tabular}{l|ccc|cccc|cccc|cccc|cc}
        \toprule
        Time & \multicolumn{15}{c|}{$t\xrightarrow{\;}$}& \\ \hline
        Method &
        \rotatebox[origin=c]{0}{GN} & \rotatebox[origin=c]{0}{SN} & \rotatebox[origin=c]{0}{IN} & \rotatebox[origin=c]{0}{DB} & \rotatebox[origin=c]{0}{GB} & \rotatebox[origin=c]{0}{MB} & \rotatebox[origin=c]{0}{ZB} & \rotatebox[origin=c]{0}{S} & \rotatebox[origin=c]{0}{Fr} & \rotatebox[origin=c]{0}{F}  & \rotatebox[origin=c]{0}{B} & \rotatebox[origin=c]{0}{C} & \rotatebox[origin=c]{0}{ET} & \rotatebox[origin=c]{0}{P} & \rotatebox[origin=c]{0}{JC}
        & Mean$\downarrow$ & Gain$\uparrow$\\\hline
        SOURCE (2021)~\citep{dosovitskiy2021vit}   & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        ROTTA (2023)~\citep{Yuan2023RobustTA}      & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        % ASR (2026)~\citep{Lim2026WhenAW}           & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        TENT (2021)~\citep{DequanWangetal2021}     & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        RPL (2021)~\citep{Rusak2021IfYD}           & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        LCOTTA (2025)~\citep{Duan2025}             & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        % RESERVOIRTTA (2025)~\citep{Vray2025ResTTA} & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        SAR (2023)~\citep{niu2023sar}              & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        RDUMB (2023)~\citep{Press2023RDumbAS}      & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        M2A (2026)~\citep{Doloriel2026Family}      & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\
        SEGA                                       & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & +100\\

        \bottomrule
    \end{tabular}%
    }%% end resizebox

\end{table*}


==> tables/cifar100c_ctta_std.tex <==
\begin{table*}[h!]
    \centering
    \small
    \caption{Fine-grained per-corruption CIFAR100-C error rates (\%) for CTTA (batch size 1) using ViT-Base. Mean is the average across 15 corruption domains, each with 10000 test samples. Gain is the relative improvement over the source model. Entries report mean and standard deviation of three runs (seeds 1, 2, 3). }
    \label{tab:cifar100c_tta_continual_std}
    \setlength\tabcolsep{6pt}
    \resizebox{\linewidth}{!}{%% relies only on graphicx, already loaded by bmvc2k
    \begin{tabular}{l|ccc|cccc|cccc|cccc|cc}
        \toprule
        Time & \multicolumn{15}{c|}{$t\xrightarrow{\;}$}& \\ \hline
        Method &
        \rotatebox[origin=c]{0}{GN} & \rotatebox[origin=c]{0}{SN} & \rotatebox[origin=c]{0}{IN} & \rotatebox[origin=c]{0}{DB} & \rotatebox[origin=c]{0}{GB} & \rotatebox[origin=c]{0}{MB} & \rotatebox[origin=c]{0}{ZB} & \rotatebox[origin=c]{0}{S} & \rotatebox[origin=c]{0}{Fr} & \rotatebox[origin=c]{0}{F}  & \rotatebox[origin=c]{0}{B} & \rotatebox[origin=c]{0}{C} & \rotatebox[origin=c]{0}{ET} & \rotatebox[origin=c]{0}{P} & \rotatebox[origin=c]{0}{JC}
        & Mean$\downarrow$ & Gain$\uparrow$\\\hline
        SOURCE (2021)~\citep{dosovitskiy2021vit}   & 55.0$\pm$0.0 & 51.5$\pm$0.0 & 26.9$\pm$0.0 & 24.0$\pm$0.0 & 60.5$\pm$0.0 & 29.0$\pm$0.0 & 21.4$\pm$0.0 & 21.1$\pm$0.0 & 25.0$\pm$0.0 & 35.1$\pm$0.0 & 11.8$\pm$0.0 & 34.8$\pm$0.0 & 43.1$\pm$0.0 & 56.0$\pm$0.0 & 35.9$\pm$0.0 & 35.4 & 0.0\\
        % ROTTA (2023)~\citep{Yuan2023RobustTA}      & 55.0$\pm$0.1 & 50.6$\pm$0.4 & 25.5$\pm$0.3 & 23.0$\pm$0.1 & 55.7$\pm$1.4 & 25.8$\pm$0.1 & 18.0$\pm$0.2 & 20.3$\pm$0.1 & 21.9$\pm$0.4 & 29.1$\pm$0.5 & 12.1$\pm$0.5 & 27.0$\pm$0.8 & 37.5$\pm$0.6 & 41.8$\pm$2.4 & 32.6$\pm$0.8 & 31.7 & +3.7\\
        % % ASR (2026)~\citep{Lim2026WhenAW}           & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100 & +100\\
        % TENT (2021)~\citep{DequanWangetal2021}     & 45.2$\pm$0.9 & 50.5$\pm$3.6 & 48.4$\pm$5.1 & 51.1$\pm$7.2 & 98.2$\pm$0.7 & 96.6$\pm$1.8 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 85.4 & -50.0\\
        % RPL (2021)~\citep{Rusak2021IfYD}           & 68.9$\pm$12.9 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 98.9$\pm$0.1 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 99.0$\pm$0.0 & 97.0 & -61.6\\
        % LCOTTA (2025)~\citep{Duan2025}             & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100 & +100\\
        % % RESERVOIRTTA (2025)~\citep{Vray2025ResTTA} & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100$\pm$10 & 100 & +100\\
        SAR (2023)~\citep{niu2023sar}              & 97.6$\pm$0.7 & 98.3$\pm$0.5 & 93.7$\pm$8.5 & 88.5$\pm$12.9 & 97.8$\pm$1.3 & 98.4$\pm$0.4 & 98.3$\pm$0.5 & 75.5$\pm$40.1 & 85.9$\pm$22.3 & 98.9$\pm$0.3 & 98.5$\pm$0.2 & 98.8$\pm$0.4 & 98.6$\pm$0.1 & 98.6$\pm$0.1 & 98.7$\pm$0.2 & 95.1 & -59.7\\
        RDUMB (2023)~\citep{Press2023RDumbAS}      & 42.1$\pm$1.8 & 38.3$\pm$0.6 & 19.8$\pm$0.5 & 21.9$\pm$0.1 & 43.2$\pm$0.9 & 24.2$\pm$1.0 & 20.2$\pm$1.7 & 19.8$\pm$0.8 & 20.3$\pm$0.3 & 26.9$\pm$1.4 & 12.1$\pm$0.1 & 19.2$\pm$0.9 & 33.2$\pm$0.7 & 25.1$\pm$1.4 & 32.1$\pm$1.8 & 26.6 & +8.8\\
        M2A (2026)~\citep{Doloriel2026Family}      & 51.8$\pm$29.7 & 49.8$\pm$34.8 & 44.0$\pm$38.9 & 45.9$\pm$37.5 & 55.3$\pm$30.9 & 46.3$\pm$37.3 & 43.4$\pm$39.4 & 44.4$\pm$38.6 & 43.6$\pm$39.1 & 45.6$\pm$37.8 & 40.7$\pm$41.2 & 43.1$\pm$39.5 & 51.3$\pm$33.8 & 46.0$\pm$37.5 & 51.1$\pm$33.9 & 46.8 & -11.4\\
        SEGA                                       & 32.6$\pm$0.8 & 29.4$\pm$1.3 & 17.7$\pm$0.5 & 23.2$\pm$1.6 & 38.7$\pm$2.1 & 23.5$\pm$0.3 & 18.4$\pm$0.6 & 18.4$\pm$0.4 & 18.4$\pm$0.1 & 21.9$\pm$0.2 & 11.6$\pm$0.1 & 16.6$\pm$0.1 & 29.9$\pm$1.5 & 20.9$\pm$0.2 & 30.9$\pm$0.3 & 23.5 & +11.9\\

        \bottomrule
    \end{tabular}%
    }%% end resizebox

\end{table*}


==> tables/cifar10c_ctta_avg.tex <==
\begin{table*}[t!]
    \centering
    \small
    \caption{Classification error rate (\%) under CTTA (batch size 1) on CIFAR10-C using ViT-Base. Mean is the average across 15 corruption domains, each with 10000 test samples. Gain is the relative improvement over the source model. Entries report mean of three runs (seeds 1, 2, 3). Fine-grained result is available in the supplementary material.}
    \label{tab:cifar10c_tta_continual_avg}
    \setlength\tabcolsep{6pt}
    \resizebox{\linewidth}{!}{%% relies only on graphicx, already loaded by bmvc2k
    \begin{tabular}{l|ccc|cccc|cccc|cccc|cc}
        \toprule
        Time & \multicolumn{15}{c|}{$t\xrightarrow{\;}$}& \\ \hline
        Method &
        \rotatebox[origin=c]{0}{GN} & \rotatebox[origin=c]{0}{SN} & \rotatebox[origin=c]{0}{IN} & \rotatebox[origin=c]{0}{DB} & \rotatebox[origin=c]{0}{GB} & \rotatebox[origin=c]{0}{MB} & \rotatebox[origin=c]{0}{ZB} & \rotatebox[origin=c]{0}{S} & \rotatebox[origin=c]{0}{Fr} & \rotatebox[origin=c]{0}{F}  & \rotatebox[origin=c]{0}{B} & \rotatebox[origin=c]{0}{C} & \rotatebox[origin=c]{0}{ET} & \rotatebox[origin=c]{0}{P} & \rotatebox[origin=c]{0}{JC}
        & Mean$\downarrow$ & Gain$\uparrow$\\\hline
        SOURCE (2021)~\citep{dosovitskiy2021vit}   & 60.1 & 53.2 & 38.3 & 19.9 & 35.5 & 22.6 & 18.6 & 12.1 & 12.7 & 22.8 & 5.3 & 49.7 & 23.6 & 24.7 & 23.1 & 28.2 & 0.0\\
        ROTTA (2023)~\citep{Yuan2023RobustTA}      & 60.9 & 56.2 & 38.4 & 18.4 & 34.2 & 17.5 & 13.1 & 10.8 & 12.1 & 14.0 & 4.2 & 21.1 & 14.8 & 27.5 & 19.8 & 24.2 & +4.0\\
        % ASR (2026)~\citep{Lim2026WhenAW}           & 67.1 & 63.5 & 38.9 & 13.5 & 43.2 & 16.6 & 14.0 & 13.5 & 15.1 & 13.3 & 4.5 & 15.5 & 23.6 & 27.9 & 28.6 & 26.6 & +1.6\\
        TENT (2021)~\citep{DequanWangetal2021}     & 59.4 & 59.0 & 30.6 & 16.7 & 35.2 & 16.8 & 12.7 & 10.7 & 12.1 & 15.6 & 4.8 & 26.7 & 16.9 & 28.6 & 20.6 & 24.4 & +3.8\\
        RPL (2021)~\citep{Rusak2021IfYD}           & 52.3 & 38.7 & 27.1 & 18.6 & 33.4 & 19.3 & 13.7 & 10.8 & 10.4 & 16.9 & 4.6 & 27.4 & 18.1 & 29.7 & 21.3 & 22.8 & +5.4\\
        LCOTTA (2025)~\citep{Duan2025}             & 57.0 & 50.2 & 37.4 & 20.1 & 35.1 & 22.8 & 18.8 & 11.8 & 12.5 & 22.9 & 5.3 & 50.5 & 23.5 & 25.0 & 22.9 & 27.7 & +0.5\\
        RES.TTA (2025)~\citep{Vray2025ResTTA} & 63.2 & 59.7 & 38.5 & 13.5 & 42.7 & 16.5 & 14.0 & 13.5 & 15.2 & 13.3 & 4.5 & 15.4 & 23.5 & 27.3 & 28.4 & 25.9 & +2.3\\
        SAR (2023)~\citep{niu2023sar}              & 55.0 & 49.4 & 38.0 & 19.5 & 35.1 & 22.3 & 18.3 & 12.0 & 12.7 & 22.4 & 5.3 & 41.7 & 23.1 & 24.2 & 23.0 & 26.9 & +1.3\\
        RDUMB (2023)~\citep{Press2023RDumbAS}      & 27.7 & 24.0 & 15.1 & 11.5 & 28.0 & 13.1 & 10.8 & 9.3 & 9.2 & 13.0 & 5.0 & 16.8 & 17.1 & 12.7 & 19.4 & 15.5 & +12.7\\
        M2A (2026)~\citep{Doloriel2026Family}      & 23.4 & 13.9 & 11.7 & 9.6 & 22.9 & 9.7 & 6.3 & 7.4 & 5.9 & 8.1 & 4.3 & 6.5 & 12.4 & 10.0 & 15.6 & 11.1 & +17.1\\
        SEGA                                       & 15.8 & 14.0 & 9.8 & 9.3 & 22.8 & 9.4 & 7.7 & 7.5 & 7.5 & 8.8 & 4.4 & 8.4 & 13.2 & 9.9 & 13.8 & 10.8 & +17.4\\

        \bottomrule
    \end{tabular}%
    }%% end resizebox

\end{table*}


==> tables/efficiency_notime.tex <==
\begin{table*}[h!]
    \centering
    \caption{Sample efficiency on ImageNet-C and CIFAR10-C using ViT-Base under CTTA (batch size 1). We use a single AMD Instinct MI200 GPU. Forward/Backward is the number of input samples used for the complete CTTA run.}
    \label{tab:sample_eff}
    \tiny
    \setlength\tabcolsep{4pt}
    \begin{adjustbox}{width=\textwidth,center=\textwidth}
    \begin{tabular}{l|ccc|c|ccc|c}
        \toprule
        \multirow{3}{*}{Method} & \multicolumn{4}{c|}{\textbf{ImageNet-C}} & \multicolumn{4}{c}{\textbf{CIFAR10-C}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9}
         & Params(\%) & Forward & Backward & Error$\downarrow$ & Params(\%) & Forward & Backward & Error$\downarrow$ \\
         \midrule
        SOURCE          & 0    & 75000  & 0     & 53.9     & 0    & 150000 & 0 & 28.2 \\
        SAR             & 0.03 & 75000  & 58569 & 46.1     & 0.03 & 150000 & 127827 & 26.9 \\
        RDUMB           & 0.05 & 75000  & 62277 & 40.8     & 0.05 & 150000 & 105079 & 15.5 \\
        M2A             & 0.03 & 75000  & 75000 & 42.4     & 0.03 & 150000 & 150000 & 11.1 \\
        SEGA            & 0.03 & 75000  & 51822 & 37.1     & 0.03 & 150000 & 99337 & 10.8 \\

        \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

==> tables/efficiency_policy.tex <==
\begin{table*}[t!]
    \centering
    \caption{Adaptation efficiency and Collapse/Drift Policy on ImageNet-C under CTTA (batch size 1) with ViT-Base on a single AMD Instinct MI200 GPU. Forward/Backward entries (e.g., 3x5000, 1x3455) denote passes per sample times number of samples per corruption domain.}
    \label{tab:efficiency_policy}
    \tiny
    \setlength\tabcolsep{4pt}
    \begin{adjustbox}{width=\textwidth,center=\textwidth}
    \begin{tabular}{l|cccc|c|cc}
        \toprule
        \multirow{3}{*}{Method} & \multicolumn{5}{c|}{\textbf{Efficiency}} & \multicolumn{2}{c}{\textbf{Collapse/Drift Policy}} \\
        \cmidrule(lr){2-6} \cmidrule(lr){7-8}
         & Param(\%) & Time(s) & Forward & Backward & Error$\downarrow$ & Recovery & Filtering \\
         \midrule
        SOURCE          & 0    & 43.8  & 1x5000  & 0    & 53.9       & None             & None \\
        SAR             & 0.03 & 163.1 & 2x5000  & 2x3904 & 46.1     & Raw Entropy      & Raw Entropy \\
        RES.TTA         & 0.03 & 236.8 & 3x5000  & 2x2805 & 42.5     & Domain Reservoir & Style Routing \\
        RDUMB           & 0.05 & 87.13 & 1x5000  & 1x4152 & 40.8     & Periodic         & Raw Entropy \\
        M2A             & 0.03 & 231.4 & 3x5000  & 1x5000 & 42.4     & None             & None \\
        SEGA            & 0.03 & 224.0 & 3x5000  & 1x3455 & 37.1     & Sensitivity      & Sensitivity \\

        \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table*}

==> tables/freshfishc_ctta_std.tex <==
\begin{table*}[h!]
    \centering
    \small
    \caption{Fine-grained per-corruption FreshFish-C error rates (\%) for CTTA (batch size 1) using ViT-Base. Mean is the average across 15 corruption domains. Gain is the relative improvement over the source model. Entries report mean and standard deviation of three runs (seeds 1, 2, 3). }
    \label{tab:freshfishc_tta_continual_std}
    \setlength\tabcolsep{6pt}
    \resizebox{\linewidth}{!}{%% relies only on graphicx, already loaded by bmvc2k
    \begin{tabular}{l|ccc|cccc|cccc|cccc|cc}
        \toprule
        Time & \multicolumn{15}{c|}{$t\xrightarrow{\;}$}& \\ \hline
        Method &
        \rotatebox[origin=c]{0}{GN} & \rotatebox[origin=c]{0}{SN} & \rotatebox[origin=c]{0}{IN} & \rotatebox[origin=c]{0}{DB} & \rotatebox[origin=c]{0}{GB} & \rotatebox[origin=c]{0}{MB} & \rotatebox[origin=c]{0}{ZB} & \rotatebox[origin=c]{0}{S} & \rotatebox[origin=c]{0}{Fr} & \rotatebox[origin=c]{0}{F}  & \rotatebox[origin=c]{0}{B} & \rotatebox[origin=c]{0}{C} & \rotatebox[origin=c]{0}{ET} & \rotatebox[origin=c]{0}{P} & \rotatebox[origin=c]{0}{JC}
        & Mean$\downarrow$ & Gain$\uparrow$\\\hline
        SOURCE (2021)~\citep{dosovitskiy2021vit}    & 24.0$\pm$0.0 & 20.7$\pm$0.0 & 21.3$\pm$0.0 & 37.6$\pm$0.0 & 27.1$\pm$0.0 & 30.1$\pm$0.0 & 20.6$\pm$0.0 & 36.3$\pm$0.0 & 35.4$\pm$0.0 & 65.3$\pm$0.0 & 12.1$\pm$0.0 & 85.6$\pm$0.0 & 10.6$\pm$0.0 & 3.7$\pm$0.0 & 3.1$\pm$0.0 & 28.9 & 0.0\\
        SAR (2023)~\citep{niu2023sar}              & 22.1$\pm$0.5 & 19.3$\pm$0.1 & 18.9$\pm$0.3 & 35.8$\pm$0.9 & 26.7$\pm$0.1 & 28.6$\pm$0.0 & 19.9$\pm$0.2 & 33.4$\pm$0.4 & 33.8$\pm$0.3 & 65.2$\pm$0.4 & 11.9$\pm$0.1 & 85.6$\pm$0.0 & 10.4$\pm$0.1 & 3.6$\pm$0.1 & 3.1$\pm$0.0 & 27.9 & +1.0\\
        RDUMB (2023)~\citep{Press2023RDumbAS}      & 20.2$\pm$2.6 & 16.9$\pm$2.1 & 17.4$\pm$1.0 & 38.8$\pm$1.2 & 26.0$\pm$0.4 & 26.8$\pm$0.1 & 19.2$\pm$1.4 & 34.7$\pm$1.0 & 35.0$\pm$0.2 & 63.3$\pm$1.8 & 11.2$\pm$0.3 & 85.6$\pm$0.0 & 8.9$\pm$0.3 & 4.0$\pm$0.5 & 3.2$\pm$0.3 & 27.4 & +1.5\\
        M2A (2026)~\citep{Doloriel2026Family}      & 16.2$\pm$0.8 & 11.5$\pm$0.1 & 9.6$\pm$0.4 & 28.2$\pm$0.7 & 20.0$\pm$0.2 & 12.1$\pm$0.8 & 10.4$\pm$0.7 & 22.0$\pm$0.5 & 21.3$\pm$0.6 & 37.7$\pm$0.5 & 8.6$\pm$0.6 & 84.1$\pm$0.1 & 15.8$\pm$0.2 & 2.3$\pm$0.5 & 2.7$\pm$0.1 & 20.2 & +8.7\\
        SEGA                                       & 10.2$\pm$0.5 & 5.8$\pm$0.4 & 3.0$\pm$0.4 & 15.3$\pm$5.1 & 8.0$\pm$0.2 & 8.3$\pm$1.1 & 6.7$\pm$0.9 & 20.2$\pm$0.6 & 9.6$\pm$0.7 & 35.0$\pm$17.8 & 6.4$\pm$0.8 & 85.4$\pm$0.2 & 6.1$\pm$1.2 & 2.3$\pm$0.3 & 1.5$\pm$0.4 & 14.9 & +14.0\\

        \bottomrule
    \end{tabular}%
    }%% end resizebox

\end{table*}


==> tables/imagenetc_ctta_avg.tex <==
\begin{table*}[t!]
    \centering
    \small
    \caption{Classification error rate (\%) under CTTA (batch size 1) on ImageNet-C using ViT-Base. Mean is the average across 15 corruption domains, each with 5000 test samples. Gain is the relative improvement over the source model. Entries report mean of three runs (seeds 1, 2, 3). Fine-grained result is available in the supplementary material.}
    \label{tab:imagenetc_tta_continual_avg}
    \setlength\tabcolsep{6pt}
    \resizebox{\linewidth}{!}{%% relies only on graphicx, already loaded by bmvc2k
    \begin{tabular}{l|ccc|cccc|cccc|cccc|cc}
        \toprule
        Time & \multicolumn{15}{c|}{$t\xrightarrow{\;}$}& \\ \hline
        Method &
        \rotatebox[origin=c]{0}{GN} & \rotatebox[origin=c]{0}{SN} & \rotatebox[origin=c]{0}{IN} & \rotatebox[origin=c]{0}{DB} & \rotatebox[origin=c]{0}{GB} & \rotatebox[origin=c]{0}{MB} & \rotatebox[origin=c]{0}{ZB} & \rotatebox[origin=c]{0}{S} & \rotatebox[origin=c]{0}{Fr} & \rotatebox[origin=c]{0}{F}  & \rotatebox[origin=c]{0}{B} & \rotatebox[origin=c]{0}{C} & \rotatebox[origin=c]{0}{ET} & \rotatebox[origin=c]{0}{P} & \rotatebox[origin=c]{0}{JC}
        & Mean$\downarrow$ & Gain$\uparrow$\\\hline
        SOURCE (2021)~\citep{dosovitskiy2021vit}   & 53.0 & 51.8 & 52.1 & 68.5 & 78.8 & 58.5 & 63.3 & 49.9 & 54.2 & 57.7 & 26.4 & 91.4 & 57.5 & 38.0 & 36.2 & 55.8 & 0.0\\
        ROTTA (2023)~\citep{Yuan2023RobustTA}      & 49.9 & 48.2 & 48.0 & 67.9 & 70.5 & 55.1 & 60.0 & 45.5 & 48.7 & 53.4 & 24.9 & 88.4 & 54.0 & 37.2 & 34.6 & 52.4 & +3.4\\
        RPL (2021)~\citep{Rusak2021IfYD}           & 46.6 & 40.6 & 40.6 & 55.7 & 55.9 & 44.6 & 51.1 & 41.0 & 42.5 & 40.9 & 23.5 & 69.0 & 64.6 & 54.9 & 54.3 & 48.4 & +7.4\\
        % ASR (2026)~\citep{Lim2026WhenAW}           & 57.9 & 54.2 & 53.8 & 58.0 & 58.4 & 51.0 & 54.7 & 48.4 & 41.5 & 35.9 & 26.9 & 51.6 & 49.4 & 43.5 & 39.8 & 48.3 & +7.5\\
        SANTA (2023)~\citep{Chakrabarty2023SATASA} & 46.0 & 43.2 & 44.6 & 58.7 & 64.4 & 47.7 & 54.1 & 40.0 & 46.6 & 41.9 & 23.3 & 89.5 & 49.1 & 34.7 & 33.5 & 47.8 & +8.0\\
        TENT (2021)~\citep{DequanWangetal2021}     & 47.4 & 41.8 & 41.7 & 57.5 & 58.4 & 45.8 & 51.5 & 40.4 & 41.9 & 41.8 & 22.5 & 54.0 & 50.2 & 31.9 & 30.9 & 43.8 & +12.0\\
        LCOTTA (2025)~\citep{Duan2025}             & 41.5 & 37.6 & 39.3 & 54.9 & 54.4 & 46.4 & 51.8 & 41.1 & 40.5 & 42.2 & 24.2 & 58.7 & 47.7 & 33.1 & 32.1 & 43.0 & +12.8\\
        RES.TTA (2025)~\citep{Vray2025ResTTA} & 41.9 & 39.5 & 39.5 & 50.0 & 47.5 & 45.0 & 49.8 & 39.0 & 39.4 & 37.3 & 21.9 & 88.7 & 38.5 & 29.3 & 29.9 & 42.5 & +13.3\\
        
        SAR (2023)~\citep{niu2023sar}              & 41.4 & 38.3 & 39.4 & 54.8 & 45.3 & 42.9 & 43.2 & 39.3 & 41.5 & 82.0 & 28.7 & 99.6 & 37.9 & 27.7 & 28.8 & 46.1 & +9.7\\
        RDUMB (2023)~\citep{Press2023RDumbAS}      & 44.0 & 42.4 & 42.4 & 49.5 & 48.2 & 43.6 & 46.2 & 35.1 & 37.9 & 37.0 & 21.6 & 69.4 & 37.4 & 27.9 & 29.5 & 40.8 & +15.0\\
        M2A (2026)~\citep{Doloriel2026Family}      & 41.2 & 35.8 & 36.2 & 49.6 & 44.9 & 38.7 & 41.1 & 34.1 & 33.7 & 32.7 & 21.2 & 64.6 & 57.4 & 51.6 & 52.5 & 42.4 & +13.4\\
        SEGA                                       & 40.5 & 37.3 & 38.3 & 47.7 & 42.1 & 38.9 & 39.4 & 31.9 & 39.7 & 36.3 & 21.1 & 55.6 & 31.6 & 27.7 & 28.4 & 37.1 & +18.7\\

        \bottomrule
    \end{tabular}%
    }%% end resizebox

\end{table*}


==> tables/mrsffiac_ctta_std.tex <==
\begin{table*}[h!]
    \centering
    \small
    \caption{Fine-grained per-corruption MRSFFIA-C error rates (\%) for CTTA (batch size 1) using ViT-Base. Mean is the average across 15 corruption domains. Gain is the relative improvement over the source model. Entries report mean and standard deviation of three runs (seeds 1, 2, 3). }
    \label{tab:mrsffiac_tta_continual_std}
    \setlength\tabcolsep{6pt}
    \resizebox{\linewidth}{!}{%% relies only on graphicx, already loaded by bmvc2k
    \begin{tabular}{l|ccc|cccc|cccc|cccc|cc}
        \toprule
        Time & \multicolumn{15}{c|}{$t\xrightarrow{\;}$}& \\ \hline
        Method &
        \rotatebox[origin=c]{0}{GN} & \rotatebox[origin=c]{0}{SN} & \rotatebox[origin=c]{0}{IN} & \rotatebox[origin=c]{0}{DB} & \rotatebox[origin=c]{0}{GB} & \rotatebox[origin=c]{0}{MB} & \rotatebox[origin=c]{0}{ZB} & \rotatebox[origin=c]{0}{S} & \rotatebox[origin=c]{0}{Fr} & \rotatebox[origin=c]{0}{F}  & \rotatebox[origin=c]{0}{B} & \rotatebox[origin=c]{0}{C} & \rotatebox[origin=c]{0}{ET} & \rotatebox[origin=c]{0}{P} & \rotatebox[origin=c]{0}{JC}
        & Mean$\downarrow$ & Gain$\uparrow$\\\hline
        SOURCE (2021)~\citep{dosovitskiy2021vit}    & 47.0$\pm$0.0 & 40.2$\pm$0.0 & 45.6$\pm$0.0 & 55.1$\pm$0.0 & 46.2$\pm$0.0 & 41.0$\pm$0.0 & 25.1$\pm$0.0 & 82.9$\pm$0.0 & 61.0$\pm$0.0 & 68.7$\pm$0.0 & 33.1$\pm$0.0 & 69.2$\pm$0.0 & 11.7$\pm$0.0 & 15.7$\pm$0.0 & 18.3$\pm$0.0 & 44.1 & 0.0\\
        SAR (2023)~\citep{niu2023sar}              & 45.2$\pm$0.7 & 38.1$\pm$1.5 & 43.7$\pm$0.5 & 56.8$\pm$0.6 & 47.1$\pm$0.1 & 41.3$\pm$0.1 & 24.9$\pm$0.0 & 82.8$\pm$0.1 & 58.5$\pm$0.5 & 69.0$\pm$0.4 & 27.2$\pm$0.6 & 69.2$\pm$0.0 & 11.6$\pm$0.0 & 15.6$\pm$0.1 & 18.4$\pm$0.1 & 43.3 & +0.8\\
        RDUMB (2023)~\citep{Press2023RDumbAS}      & 48.6$\pm$0.2 & 41.0$\pm$0.5 & 46.4$\pm$0.2 & 56.3$\pm$0.2 & 46.6$\pm$2.3 & 40.9$\pm$1.4 & 24.7$\pm$0.5 & 82.9$\pm$0.0 & 59.7$\pm$1.6 & 68.8$\pm$0.1 & 31.8$\pm$0.4 & 69.2$\pm$0.0 & 11.2$\pm$0.2 & 15.8$\pm$0.6 & 18.8$\pm$0.2 & 44.2 & -0.1\\
        M2A (2026)~\citep{Doloriel2026Family}      & 31.3$\pm$0.7 & 32.2$\pm$0.5 & 26.3$\pm$0.3 & 62.7$\pm$1.0 & 66.4$\pm$0.0 & 66.4$\pm$0.0 & 66.4$\pm$0.0 & 66.4$\pm$0.1 & 66.4$\pm$0.0 & 66.4$\pm$0.0 & 66.4$\pm$0.1 & 61.6$\pm$2.9 & 66.2$\pm$0.2 & 66.4$\pm$0.0 & 66.4$\pm$0.0 & 58.5 & -14.4\\
        SEGA                                       & 38.7$\pm$3.8 & 35.1$\pm$13.4 & 36.7$\pm$13.8 & 42.0$\pm$10.0 & 41.2$\pm$10.5 & 38.4$\pm$14.7 & 42.0$\pm$5.6 & 53.1$\pm$16.4 & 45.3$\pm$9.1 & 68.3$\pm$1.8 & 28.4$\pm$13.4 & 69.2$\pm$0.0 & 11.6$\pm$0.8 & 17.1$\pm$5.5 & 19.0$\pm$5.6 & 39.1 & +5.0\\

        \bottomrule
    \end{tabular}%
    }%% end resizebox

\end{table*}

